The Impact of Host Galaxy Properties on Supernova Classification with Hierarchical Labels

With the advent of the Vera C. Rubin Observatory, the discovery rate of supernovae (SNe) will surpass the rate of SNe with real time spectroscopic followup by three orders of magnitude. Accurate photometric classifiers are essential to both select interest events for followup in real time and for archival population-level studies. In this work, we investigate the impact of observable host galaxy information on the classification of SNe, both with and without additional light curve and redshift information. We find that host galaxy information alone can successfully isolate relatively pure (>90%) samples of Type Ia SNe with or without redshift information. With redshift information, we can additionally produce somewhat pure (>70%) samples of Type II SNe and superluminous supernovae. Additionally with redshift information, host galaxy properties do not significantly improve the accuracy of SN classification when paired with complete light curves. In the absence of redshift information, however, galaxy properties significantly increase the accuracy of photometric classification. As a part of this analysis, we present the first formal application of a new objective function, the weighted hierarchical cross-entropy, to the problem of supernova classification. This objective function more naturally accounts for the hierarchical nature of supernova classes and, more broadly, transients. Finally, we present a new set of SN classifications for the Pan-STARRS Medium Deep Survey of SNe that lack spectroscopic redshift, increasing the full photometric sample to >4400 events.

==> table.tex <==
\begin{deluxetable*}{ccccccccccc}
\tabletypesize{\footnotesize}
\tablecolumns{11}
\tablecaption{ Cross-correlation Fit Details \label{table:results1}}
\tablehead{
\colhead{-} & \colhead{GalLC} & \colhead{GalLC0.8} & \colhead{Gallc noz} & \colhead{Gallcnoz0.8} & \colhead{Gal} & \colhead{Gal0.8} &\colhead{LC} & \colhead{LC0.8} & \colhead{LCnoz} & \colhead{LCnoz0.8} }
 \startdata
SLSN Accuracy & 0.98 (0.01) &  0.98 (0.01) &  0.95 (0.01) &  0.96 (0.01) &  0.87 (0.01) &  0.76 (0.02) &  0.98 (0.01) &  0.99 (0.01) &  0.93 (0.01) &  0.97 (0.01)\\
SLSN Purity & 0.60 (0.05) &  0.67 (0.04) &  0.22 (0.04) &  0.26 (0.04) &  0.09 (0.01) &  0.09 (0.04) &  0.71 (0.04) &  0.79 (0.06) &  0.12 (0.03) &  0.00 (0.14)\\
SLSN Completeness & 0.67 (0.03) &  0.75 (0.05) &  0.33 (0.08) &  0.45 (0.09) &  0.40 (0.05) &  0.60 (0.06) &  0.80 (0.03) &  0.85 (0.03) &  0.20 (0.06) &  nan (nan)\\
II Accuracy & 0.90 (0.01) &  0.94 (0.01) &  0.88 (0.01) &  0.93 (0.01) &  0.78 (0.01) &  0.91 (0.02) &  0.91 (0.01) &  0.97 (0.01) &  0.84 (0.01) &  0.94 (0.01)\\
II Purity & 0.70 (0.02) &  0.83 (0.02) &  0.70 (0.02) &  0.77 (0.03) &  0.36 (0.01) &  0.67 (0.11) &  0.80 (0.03) &  0.94 (0.03) &  0.56 (0.04) &  0.89 (0.08)\\
II Completeness & 0.70 (0.02) &  0.77 (0.03) &  0.57 (0.03) &  0.54 (0.02) &  0.40 (0.02) &  0.33 (0.11) &  0.66 (0.02) &  0.76 (0.03) &  0.46 (0.02) &  0.43 (0.05)\\
IIn Accuracy & 0.94 (0.01) &  0.96 (0.01) &  0.92 (0.01) &  0.96 (0.01) &  0.81 (0.01) &  0.90 (0.02) &  0.95 (0.01) &  0.97 (0.01) &  0.92 (0.01) &  0.98 (0.01)\\
IIn Purity & 0.35 (0.05) &  0.44 (0.09) &  0.22 (0.02) &  0.30 (0.08) &  0.07 (0.01) &  0.11 (0.10) &  0.42 (0.05) &  0.62 (0.07) &  0.25 (0.04) &  0.50 (0.29)\\
IIn Completeness & 0.38 (0.07) &  0.42 (0.08) &  0.29 (0.03) &  0.28 (0.09) &  0.25 (0.05) &  0.33 (0.15) &  0.46 (0.07) &  0.50 (0.07) &  0.38 (0.06) &  0.25 (0.17)\\
Ia Accuracy & 0.89 (0.01) &  0.94 (0.01) &  0.86 (0.01) &  0.93 (0.01) &  0.61 (0.01) &  0.70 (0.02) &  0.90 (0.01) &  0.97 (0.01) &  0.83 (0.01) &  0.95 (0.01)\\
Ia Purity & 0.95 (0.01) &  0.96 (0.01) &  0.92 (0.01) &  0.94 (0.01) &  0.88 (0.01) &  0.94 (0.02) &  0.96 (0.01) &  0.97 (0.01) &  0.94 (0.01) &  0.95 (0.01)\\
Ia Completeness & 0.90 (0.01) &  0.96 (0.01) &  0.88 (0.01) &  0.96 (0.01) &  0.52 (0.01) &  0.66 (0.02) &  0.90 (0.01) &  0.99 (0.01) &  0.82 (0.01) &  1.00 (0.01)\\
Ibc Accuracy & 0.93 (0.01) &  0.96 (0.01) &  0.93 (0.01) &  0.97 (0.01) &  0.88 (0.01) &  0.90 (0.01) &  0.89 (0.01) &  0.98 (0.01) &  0.89 (0.01) &  0.99 (0.01)\\
Ibc Purity & 0.23 (0.02) &  0.32 (0.05) &  0.23 (0.03) &  0.35 (0.15) &  0.09 (0.02) &  0.00 (0.08) &  0.15 (0.02) &  0.33 (0.15) &  0.14 (0.02) &  nan (nan)\\
Ibc Completeness & 0.47 (0.04) &  0.50 (0.07) &  0.42 (0.06) &  0.39 (0.18) &  0.26 (0.04) &  0.00 (0.17) &  0.42 (0.06) &  0.50 (0.13) &  0.42 (0.05) &  0.00 (0.25)\\
Avg. Accuracy & 0.93 (0.01) &  0.95 (0.01) &  0.91 (0.01) &  0.95 (0.01) &  0.79 (0.01) &  0.83 (0.01) &  0.93 (0.01) &  0.98 (0.01) &  0.88 (0.01) &  0.97 (0.01)\\
Avg. Purity & 0.56 (0.02) &  0.64 (0.02) &  0.46 (0.01) &  0.53 (0.04) &  0.30 (0.01) &  0.36 (0.03) &  0.61 (0.01) &  0.73 (0.04) &  0.40 (0.01) &  nan (nan)\\
Avg. Completeness & 0.62 (0.02) &  0.68 (0.02) &  0.50 (0.02) &  0.52 (0.04) &  0.37 (0.02) &  0.39 (0.05) &  0.65 (0.02) &  0.72 (0.03) &  0.46 (0.02) &  nan (nan)\\
W. Accuracy & 0.90 (0.01) &  0.94 (0.01) &  0.87 (0.01) &  0.93 (0.01) &  0.66 (0.01) &  0.74 (0.01) &  0.91 (0.01) &  0.97 (0.01) &  0.84 (0.01) &  0.95 (0.01)\\
W. Purity & 0.84 (0.01) &  0.89 (0.01) &  0.81 (0.01) &  0.88 (0.01) &  0.70 (0.01) &  0.78 (0.02) &  0.87 (0.01) &  0.94 (0.01) &  0.79 (0.01) &  nan (nan)\\
W. Completeness & 0.82 (0.01) &  0.89 (0.01) &  0.77 (0.01) &  0.88 (0.01) &  0.47 (0.01) &  0.59 (0.02) &  0.82 (0.01) &  0.94 (0.01) &  0.70 (0.01) &  nan (nan)\\
II Accuracy & 0.87 (0.01) &  0.91 (0.01) &  0.86 (0.01) &  0.89 (0.01) &  0.63 (0.01) &  0.74 (0.02) &  0.88 (0.01) &  0.94 (0.01) &  0.83 (0.01) &  0.91 (0.01)\\
II Purity & 0.70 (0.02) &  0.80 (0.02) &  0.69 (0.03) &  0.75 (0.03) &  0.32 (0.01) &  0.44 (0.05) &  0.75 (0.02) &  0.88 (0.02) &  0.62 (0.02) &  0.84 (0.02)\\
II Completeness & 0.71 (0.02) &  0.77 (0.02) &  0.65 (0.03) &  0.70 (0.02) &  0.63 (0.02) &  0.68 (0.07) &  0.70 (0.01) &  0.82 (0.02) &  0.67 (0.02) &  0.75 (0.02)\\
Ia Accuracy & 0.89 (0.01) &  0.93 (0.01) &  0.86 (0.01) &  0.91 (0.01) &  0.57 (0.01) &  0.63 (0.02) &  0.90 (0.01) &  0.96 (0.01) &  0.82 (0.01) &  0.94 (0.01)\\
Ia Purity & 0.95 (0.01) &  0.96 (0.01) &  0.92 (0.01) &  0.94 (0.01) &  0.90 (0.01) &  0.94 (0.02) &  0.96 (0.01) &  0.97 (0.01) &  0.94 (0.01) &  0.95 (0.01)\\
Ia Completeness & 0.90 (0.01) &  0.95 (0.01) &  0.88 (0.01) &  0.93 (0.01) &  0.44 (0.01) &  0.52 (0.03) &  0.90 (0.01) &  0.98 (0.01) &  0.80 (0.01) &  0.97 (0.01)\\
SE Accuracy & 0.91 (0.01) &  0.93 (0.01) &  0.88 (0.01) &  0.92 (0.01) &  0.77 (0.01) &  0.72 (0.03) &  0.88 (0.01) &  0.96 (0.01) &  0.84 (0.01) &  0.93 (0.01)\\
SE Purity & 0.35 (0.02) &  0.44 (0.04) &  0.26 (0.04) &  0.31 (0.07) &  0.13 (0.01) &  0.18 (0.03) &  0.30 (0.02) &  0.64 (0.06) &  0.19 (0.01) &  0.24 (0.05)\\
SE Completeness & 0.56 (0.03) &  0.59 (0.02) &  0.43 (0.05) &  0.42 (0.09) &  0.44 (0.04) &  0.60 (0.06) &  0.56 (0.04) &  0.65 (0.04) &  0.44 (0.03) &  0.36 (0.08)\\
Avg. Accuracy & 0.89 (0.01) &  0.92 (0.01) &  0.87 (0.01) &  0.91 (0.01) &  0.66 (0.01) &  0.70 (0.01) &  0.89 (0.01) &  0.95 (0.01) &  0.83 (0.01) &  0.93 (0.01)\\
Avg. Purity & 0.67 (0.01) &  0.73 (0.02) &  0.63 (0.02) &  0.67 (0.02) &  0.45 (0.01) &  0.52 (0.02) &  0.67 (0.01) &  0.83 (0.02) &  0.58 (0.01) &  0.68 (0.02)\\
Avg. Completeness & 0.72 (0.01) &  0.77 (0.01) &  0.65 (0.02) &  0.69 (0.03) &  0.51 (0.01) &  0.60 (0.03) &  0.72 (0.01) &  0.82 (0.02) &  0.64 (0.01) &  0.69 (0.03)\\
W. Accuracy & 0.89 (0.01) &  0.93 (0.01) &  0.86 (0.01) &  0.91 (0.01) &  0.60 (0.01) &  0.66 (0.01) &  0.89 (0.01) &  0.96 (0.01) &  0.82 (0.01) &  0.94 (0.01)\\
W. Purity & 0.85 (0.01) &  0.89 (0.01) &  0.83 (0.01) &  0.87 (0.01) &  0.72 (0.01) &  0.76 (0.02) &  0.87 (0.01) &  0.93 (0.01) &  0.82 (0.01) &  0.91 (0.01)\\
W. Completeness & 0.83 (0.01) &  0.89 (0.01) &  0.80 (0.01) &  0.86 (0.01) &  0.49 (0.01) &  0.56 (0.03) &  0.83 (0.01) &  0.93 (0.01) &  0.75 (0.01) &  0.90 (0.01)\\
Ia Accuracy & 0.91 (0.01) &  0.92 (0.01) &  0.88 (0.01) &  0.90 (0.01) &  0.68 (0.01) &  0.56 (0.01) &  0.92 (0.01) &  0.93 (0.01) &  0.87 (0.01) &  0.86 (0.01)\\
Ia Purity & 0.84 (0.01) &  0.84 (0.01) &  0.80 (0.02) &  0.80 (0.02) &  0.46 (0.01) &  0.46 (0.01) &  0.85 (0.01) &  0.85 (0.01) &  0.76 (0.02) &  0.76 (0.02)\\
Ia Completeness & 0.83 (0.01) &  0.90 (0.01) &  0.77 (0.02) &  0.87 (0.01) &  0.66 (0.01) &  0.96 (0.02) &  0.87 (0.01) &  0.94 (0.01) &  0.80 (0.01) &  0.93 (0.01)\\
CC Accuracy & 0.91 (0.01) &  0.92 (0.01) &  0.88 (0.01) &  0.90 (0.01) &  0.68 (0.01) &  0.56 (0.01) &  0.92 (0.01) &  0.93 (0.01) &  0.87 (0.01) &  0.86 (0.01)\\
CC Purity & 0.93 (0.01) &  0.96 (0.01) &  0.91 (0.01) &  0.94 (0.01) &  0.83 (0.01) &  0.94 (0.02) &  0.95 (0.01) &  0.97 (0.01) &  0.92 (0.01) &  0.95 (0.01)\\
CC Completeness & 0.94 (0.01) &  0.93 (0.01) &  0.92 (0.01) &  0.91 (0.01) &  0.69 (0.01) &  0.34 (0.02) &  0.94 (0.01) &  0.93 (0.01) &  0.90 (0.01) &  0.83 (0.01)\\
Avg. Accuracy & 0.91 (0.01) &  0.92 (0.01) &  0.88 (0.01) &  0.90 (0.01) &  0.68 (0.01) &  0.56 (0.01) &  0.92 (0.01) &  0.93 (0.01) &  0.87 (0.01) &  0.86 (0.01)\\
Avg. Purity & 0.89 (0.01) &  0.90 (0.01) &  0.85 (0.01) &  0.87 (0.01) &  0.65 (0.01) &  0.70 (0.01) &  0.90 (0.01) &  0.91 (0.01) &  0.84 (0.01) &  0.86 (0.01)\\
Avg. Completeness & 0.89 (0.01) &  0.92 (0.01) &  0.85 (0.01) &  0.89 (0.01) &  0.68 (0.01) &  0.65 (0.01) &  0.91 (0.01) &  0.93 (0.01) &  0.85 (0.01) &  0.88 (0.01)\\
W. Accuracy & 0.91 (0.01) &  0.92 (0.01) &  0.88 (0.01) &  0.90 (0.01) &  0.68 (0.01) &  0.56 (0.01) &  0.92 (0.01) &  0.93 (0.01) &  0.87 (0.01) &  0.86 (0.01)\\
W. Purity & 0.91 (0.01) &  0.92 (0.01) &  0.88 (0.01) &  0.90 (0.01) &  0.73 (0.01) &  0.76 (0.01) &  0.92 (0.01) &  0.93 (0.01) &  0.87 (0.01) &  0.88 (0.01)\\
W. Completeness & 0.91 (0.01) &  0.92 (0.01) &  0.88 (0.01) &  0.90 (0.01) &  0.68 (0.01) &  0.57 (0.01) &  0.92 (0.01) &  0.93 (0.01) &  0.87 (0.01) &  0.86 (0.01)\\
\enddata
\end{deluxetable*}

